Intrusion Detection based on Federated Learning: a systematic review

The evolution of cybersecurity is undoubtedly associated and intertwined with the development and improvement of artificial intelligence (AI). As a key tool for realizing more cybersecure ecosystems, Intrusion Detection Systems (IDSs) have evolved tremendously in recent years by integrating machine learning (ML) techniques for the detection of increasingly sophisticated cybersecurity attacks hidden in big data. However, these approaches have traditionally been based on centralized learning architectures, in which data from end nodes are shared with data centers for analysis. Recently, the application of federated learning (FL) in this context has attracted great interest to come up with collaborative intrusion detection approaches where data does not need to be shared. Due to the recent rise of this field, this work presents a complete, contemporary taxonomy for FL-enabled IDS approaches that stems from a comprehensive survey of the literature in the time span from 2018 to 2022. Precisely, our discussion includes an analysis of the main ML models, datasets, aggregation functions, as well as implementation libraries, which are employed by the proposed FL-enabled IDS approaches. On top of everything else, we provide a critical view of the current state of the research around this topic, and describe the main challenges and future directions based on the analysis of the literature and our own experience in this area.

==> analysisv2.tex <==
\section{Analysis} \label{sec:analysis}\textcolor{red}{\textbf{Jose, Vasilis, Giorgos}}

This section provides an analysis of existing proposals that use FL for IDS. Potential classification aspects:

\begin{itemize}
    \item Attacks:
    \item Dataset:
    \item ML model (supervised/unsupervised)
    \item Aggregation function
    \item Training device type?
    \item Implementation/Evaluation aspects, including FL library, number of rounds, FL clients, accuracy, recall, F1-score and precision, use of non-iid data??
\end{itemize}

To include a figure with the scheme based on such aspects. 

\hl{This needs to be decided: how to organize this section to describe the papers}

%\subsection{Supervised learning based approaches}

%\subsection{Unsupervised learning based approaches}

\begin{table*}[]
\tiny
\centering
\begin{tabular}{C{1.2cm}C{0.2cm}C{1.2cm}C{1.2cm}C{1.2cm}C{1.2cm}C{1.2cm}C{1.2cm}C{1.2cm}C{1.2cm}C{1.2cm}C{1.2cm}}

\textbf{Reference} & \textbf{Year} & \textbf{Dataset} & \textbf{ML Model} & \textbf{FL implementation} & \textbf{Aggregation function} & \textbf{Training parties} & \textbf{Training rounds/epochs} & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} & \textbf{F-1 score}\\ \hline \hline

\cite{schneible2017anomaly} & 2017 & KDD Cup 99 \cite{tavallaee2009detailed} & Autoencoders & -- & FedAvg & 3 & 100/2-300 & -- & -- & -- & 0.9444\\ \hline

\cite{preuveneers2018chained} & 2018 & CICIDS2017 & Autoencoders  & Based on Keras, Deeplearning4j and Spring Boot 2.0 & FedAvg & 2-12 & 1/1-50 & 0.97 & -- & -- & -- \\ \hline

%Jose: This is a MSc thesis and results are quite unclear
%\cite{schneble2018federated} & 2018 & MIMIC-III \cite{johnson2016mimic} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline

\cite{chen2019network} & 2019 & KDD Cup 99 & DAGMM \cite{zong2018deep} & -- & FedAvg & 2 & 1-60/1 & -- & 0.4532-0.7447 & 0.9769-0.9927 & 0.6-0.87\\ \hline

\cite{schneble2019attack} & 2019 & MIMIC-III \cite{johnson2016mimic} & Feedforward NN & Based on Matlab and scikit-learn & FedAvg & 1-8 & 8/1 & 0.99-0994 & -- & -- & -- \\ \hline

\cite{nguyen2019diot} & 2019 & Generated & Gated recurrent Unit (GRU) & Based on Flask and Keras & FedAvg & 1-15 & 3/17 & \hl{TBD}& \hl{TBD} & \hl{TBD} & \hl{TBD}\\ \hline

\cite{cetin2019federated} & 2019 & AWID & Stacked Autoencoders & LEAF & FedAvg & 933 & 1-20/1 & $\approx$ 0.9 & -- & -- & --\\ \hline

%Jose: this paper does not provide results
%\cite{wang2019machine} & 2019 & KDD Cup 99 & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline

\cite{zhao2019multi} & 2019 & CICIDS2017, ISCXVPN2016, ISCXTor2016 & Multi-task NN & Based on Pytorch & FedAvg & ? & ?/? & \hl{TBD} & \hl{TBD} &\hl{TBD} & \hl{TBD}\\ \hline

\cite{akbariprivpkt} & 2019 & ISCXVPN2016 & Convolutional NN & Based on TensorFlow-Keras & FedAvg & 10 & 15 & \hl{TBD}& \hl{TBD} & \hl{TBD} & \hl{TBD}\\ \hline

%\cite{yang2019tradeoff} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline

\cite{regan2020federated} & 2020 & N-BaIoT & Autoencoders & PySyft & FedAvg? & 9 & 50 epochs (rounds) &  \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline

\cite{hei2020trusted} & 2020 & KDD CUP 99 & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline

\cite{sun2020adaptive} & 2020 & Generated & Convolutional NN & ? & FedAvg & 20 & 1-60/1-5 & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline

%\cite{leeae} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline

%\cite{wang2020intrusion} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline


\cite{khoa2020collaborative} & 2020 & KDD, NSL-KDD, UNSW-NB15, N-BaIoT & Deep belief network & -- & FedAvg & \hl{TBD} & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline

%Jose: actually this one is not about intrusion but only anomaly detection
%\cite{liu2020deep} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline

\cite{li2020distributed} & 2020 & Generated \cite{stin_dataset} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline


\cite{weinger2020enhancing} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline

\cite{zhao2020intelligent} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline

\cite{fan2020iotdefender} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline

\cite{zhao2020network} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline

\cite{cetin2020wireless} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline

\cite{nguyen2020poisoning} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline

\cite{al2020federated} & NSL-KDD & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline

\cite{aliyu2021blockchain} & OTIDS & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline

 \cite{FLEAM} & Simulated traffic & GRU & - & FedAvg & - & - & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline

\cite{BFL-CIDS} & KDDCup99 & MLP, DT, SVM, RF & - & FedAvg & - & 50 & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline

\cite{FLMimicIDS}  & NSL-KDD & MLPs & TensorFlow, Keras & FedAvg  & 10 & 20 & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline

\cite{rahman2020internet} & NSL-KDD & NN & - & FedAvg & 4 & 1-5 & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline

\cite{FLHeteCohort} & CSE-CIC-IDS2018 & NN & TensorFlow & FedAvg & 1-50 & 10000 & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline

\cite{BNNSIDFL} & CICIDS2017, ISCX Botnet 2014 & Binarized NN & TensorFlow & signSGD & - & - & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline

\cite{LocKedge} &  BoT-IoT & NN & - & FedAvg & 4 & 1000 & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline 

\cite{rey2021federated} &  N-BaIoT & MLP, autoencoders & own library \cite{fediotguard} & FedAvg, Coordinate-wise median/trimmed mean & 8 & 1-29 & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline



\cite{campos2021evaluating} & ToN\_IoT & Logistic regression & IBMFL & FedAvg, Fed+ & 4/10 & 1-300 & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline 



\cite{chatterjee2021federated} & NSL-KDD & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline

\cite{chen2020intrusion} & KDDCUP-99, WSN-DS, CICIDS2017 & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline

\cite{gaussian2020network} & KDDCUP-99 & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline



\cite{kim2020collaborative} & NSL-KDD & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline

\cite{li2020deepfed} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline

\cite{li2020detecting} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline

\cite{li2020distributed} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline

\cite{liu2021blockchain} & KDDCup99 & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline

\cite{mothukuri2021federated} & Modbus dataset & GRU & Pytorch/PySyft & FedAvg & - & 1-40 & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline


\cite{nguyen2021federated} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline

\cite{otoum2021federated} & CICIDS2017 & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline

\cite{popoola2021federated} & Bot-IoT & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline

\cite{qin2020line} & CICIDS2017, ISCX Botnet 2014 & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline

\cite{rahman2020internet} & NSL-KDD & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline

\cite{saadat2021hierarchical} & NSL-KDD & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline

\cite{shi2021data} & UNSW-NB15, CICIDS2018 & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline

\cite{shingi2021segmented} & CIDDS-001, CIDDS-002 & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline



\cite{wang2021non} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline

\cite{xie2021improved} & AWID & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline

\cite{zhao2020network} & UNSW-NB15 & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD} & \hl{TBD}& \hl{TBD} & \hl{TBD}\\ \hline

\end{tabular}
\caption{Classification of existing works on FL-enabled IDS}
\label{tab:taxonomy_table}
\end{table*}

Conclusions about the analysis to be further discussed

\begin{itemize}
    \item A significant number of proposed FL-enabled IDS approaches are based on obsolete datasets, which do not consider existing networking technologies and related attacks
\end{itemize}

\subsection{Datasets}
We will analyze which dataset is more used with a graph and discussion

\subsection{Models}
We will analyze which ML is more used with a graph and discussion


\subsection{Aggregation}
We will analyze which ML is more used with a graph and discussion

==> reinforcement-table.tex <==
\onecolumn
\begin{center}
\fontsize{6}{11}\selectfont{
\begin{longtable}{C{0.5cm}C{1cm}C{1.5cm}C{1.5cm}C{1.5cm}C{1.5cm}C{1.5cm}C{1.5cm}C{1.5cm}C{0.8cm}C{0.8cm}C{2.5cm}C{1.2cm}}
\caption{Classification of existing works on FL-enabled IDS based on reinforcement models}
\label{tab:super_taxonomy_long_table} \\

%\textbf{Training rounds/epochs}
\hline 
\textbf{Ref.} & \textbf{Year} & \textbf{Network Architecture} & \textbf{Data Availability} & \textbf{Data Partitioning} & \textbf{Dataset} & \textbf{ML Model} & \textbf{Aggregation function} & \textbf{FL implementation}  & \textbf{Training parties} & \textbf{Training rounds} & \textbf{Evaluation metrics} & \textbf{Citations (as of D/M/2022)} \\
\hline 
\endfirsthead

\multicolumn{12}{c}%
%{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
{\tablename\ \thetable{} -- continued from previous page} \\
\hline 
\textbf{Ref.} & \textbf{Year} & \textbf{Network Architecture} & \textbf{Data Availability} & \textbf{Data Partitioning} & \textbf{Dataset} & \textbf{ML Model} & \textbf{Aggregation function} & \textbf{FL implementation}  & \textbf{Training parties} & \textbf{Training rounds} & \textbf{Evaluation metrics}  \\
\hline 
\endhead

\hline \multicolumn{13}{c}{{Continued on next page}} \\ \hline
\endfoot

\hline \hline
\endlastfoot


%Federated learning empowered end-edge-cloud cooperation for 5G HetNet security 
\cite{wei2021federated} & 2021 & Cross-device & Horizontal & Centralized & CICIDS2017 & Deep Q-networks  & Based on FedAvg & Pytorch & 1-10 & 1-4/1-1000 & Error rate, reward  \\ \hline

%Federated deep reinforcement learning for traffic monitoring in sdn-based iot networks 
\cite{nguyen2021federated} & 2021 & Cross-device & Horizontal & Centralized & \hl{?} & Double Deep Q Networks (DDQN), SOM  & FedAvg & TFF & 6 & 1-200/1 & Reward, loss, communication overhead  \\ \hline


\end{longtable}
}
\end{center}
\twocolumn
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%55
%\end{tabular}
%\caption{Classification of existing works on FL-enabled IDS based on supervised models}
%\label{tab:super_taxonomy_table}
%\end{table*}
%\end{landscape}





==> superv-table.tex <==
%\begin{table*}[]
%\tiny
%\centering
%\begin{tabular}{C{0.8cm}C{0.8cm}C{1.2cm}C{1.2cm}C{1.5cm}C{1.2cm}C{1.2cm}C{1.2cm}C{3cm}C{1.2cm}}

%\textbf{Reference} & \textbf{Year} & \textbf{Dataset} & \textbf{ML Model} & \textbf{Aggregation function} & \textbf{FL implementation}  & \textbf{Training parties} & \textbf{Training rounds/epochs} & \textbf{Evaluation metrics} & \textbf{Citations (as of D/M/2022)} \\ \hline \hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{landscape}



\onecolumn
\begin{center}
\tiny
%\fontsize{6}{11}\selectfont{
\begin{longtable}{C{0.4cm}C{0.4cm}C{1.2cm}C{1.2cm}C{1.2cm}C{1.5cm}C{1.5cm}C{1.5cm}C{1.5cm}C{0.8cm}C{0.8cm}C{2.5cm}}
\caption{Classification of existing works on FL-enabled IDS based on supervised models}
\label{tab:super_taxonomy_long_table} \\

%\textbf{Training rounds/epochs}
\hline 
\textbf{Ref.} & \textbf{Year} & \textbf{Network Architecture} & \textbf{Data Availability} & \textbf{Data Partitioning} & \textbf{Dataset} & \textbf{ML Model} & \textbf{Aggregation function} & \textbf{FL implementation}  & \textbf{Training parties} & \textbf{Training rounds} & \textbf{Evaluation metrics} %& \textbf{Citations (as of D/M/2022)} 
\\
\hline 
\endfirsthead

\multicolumn{12}{c}%
%{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
{\tablename\ \thetable{} -- continued from previous page} \\
\hline 
\textbf{Ref.} & \textbf{Year} & \textbf{Network Architecture} & \textbf{Data Availability} & \textbf{Data Partitioning} & \textbf{Dataset} & \textbf{ML Model} & \textbf{Aggregation function} & \textbf{Implementation}  & \textbf{Training parties} & \textbf{Training rounds} & \textbf{Evaluation metrics} %\textbf{Citations (as of D/M/2022)} 
\\
\hline 
\endhead

\hline \multicolumn{12}{c}{{Continued on next page}} \\ \hline
\endfoot

\hline \hline
\endlastfoot

%DÏoT: A federated self-learning anomaly detection system for IoT 
\cite{nguyen2019diot} & 2019 & Cross-device & Horizontal & Centralized & Generated & GRU & FedAvg & Based on Flask and Keras  & 2-15 & 3/51 & FPR, TPR, time  \\ \hline

%Multi-task network anomaly detection using federated learning 
\cite{zhao2019multi} & 2019 & Cross-device & Vertical & Centralized & CICIDS2017, ISCXVPN2016, ISCXTor2016 & NN (multi-task)  & FedAvg & Based on Pytorch & - & - & Accuracy, precision, recall, training time \\ \hline

%Collaborative Learning Based Effective Malware Detection System
\cite{singh2020collaborative} & 2020 & Cross-device & Horizontal & Centralized & Microsoft Malware \cite{ronen2018microsoft} & CNN, Auxiliary Classifier GAN & FedAvg & TensorFlow Federated  & 5 & 50-100/10 & Accuracy, precision, recall, F1   \\ \hline

%Distributed Network Intrusion Detection System in Satellite-Terrestrial Integrated Networks Using Federated Learning
\cite{li2020distributed} & 2020 & Cross-device & Horizontal & Centralized & Generated \cite{stin_dataset} & CNN  & - & TensorFlow Federated & - & 1-8/1 & FPR, TPR, training time, CPU use   \\ \hline

%Intrusion Detection for Wireless Edge Networks Based on Federated Learning 
\cite{chen2020intrusion} & 2020 & Cross-device & Horizontal & Centralized & WSN-DS, KDDCup99, CICIDS2017 & GRU-SVM  & FedAvg, CMFL and based on FedAvg & PySyft & 10-50 & 1-50/1 & Accuracy, FAR, recall   \\ \hline

%Network Anomaly Detection Using Federated Learning and Transfer Learning 
\cite{zhao2020network} & 2020  & Cross-device & Transfer Learning & Centralized & UNSW-NB15 & DNN  & FedAvg & - & 10 & -/- & Accuracy, precision, recall   \\ \hline


%Federated learning-based cognitive detection of jamming attack in flying ad-hoc network
\cite{mowla2019federated} & 2020 & Cross-device & Horizontal & Centralized & CRAWDAD \cite{crawdad} & NN  & FedAvg & - & 6 & 1-10/25 & Accuracy  \\ \hline

%Federated Mimic Learning for Privacy Preserving Intrusion Detection 
\cite{al2020federated} & 2020 & Cross-device & Horizontal & Centralized &  NSL-KDD & MLP  & FedAvg & TensorFlow, Keras & 10 & 20/10 & Accuracy, precision, recall, F1-score &  \\ \hline

%Line-speed and scalable intrusion detection at the network edge via federated learning 
\cite{qin2020line} & 2020 & Cross-device & Horizontal & Centralized & CICIDS2017, ISCX Botnet 2014 & BNN & signSGD & TensorFlow, Keras & 2-8 & -/- & Accuracy, precision, recall, F1-score, latency, overhead &  \\ \hline

%Intrusion Detection with Segmented Federated Learning for Large-Scale Multiple LANs 
\cite{sun2020intrusion} & 2020 & Cross-device & Horizontal & Centralized & Generated & CNN & FedAvg & - & 20 & 1-60/1 & Accuracy, precision, recall, F1-score &  \\ \hline

%A Privacy-Preserving Federated Learning System for Android Malware Detection Based on Edge Computing
\cite{hsu2020privacy} & 2020 & Cross-device & Horizontal, Vertical & Centralized &  Generated & SVM & FedAvg & Based on Python & 2-30 & 10/30 & Accuracy, precision, recall, FPR, F1-score &  \\ \hline

%Intelligent intrusion detection based on federated learning aided long short-term memory 
\cite{zhao2020intelligent} & 2020 & Cross-device & Horizontal & Centralized & SEA \cite{schonlau2001computer} & LSTM, CNN  & FedAvg & TensorFlow, Keras & 4 & 1-50/1 & Accuracy, precision, recall, F1-score, latency, overhead &  \\ \hline

%Internet of things intrusion detection: Centralized, on-device, or federated learning? 
\cite{rahman2020internet} & 2020 & Cross-device & Horizontal & Centralized & NSL-KDD & NN  & FedAvg & - & 4 & 1-5/1 & Accuracy &  \\ \hline

%Federated deep payload classification for industrial internet with cloud-edge architecture 
\cite{zhou2020federated} & 2020 & Cross-device & Horizontal & Centralized & \cite{igbe2017deterministic, morris2014industrial} & CNN  & FedAvg & Based on Pytorch & 2-10 & 5/20 & Accuracy &  \\ \hline

%Iotdefender: A federated transfer learning intrusion detection framework for 5G IoT 
\cite{fan2020iotdefender} & 2020 & Cross-device & Transfer Learning & Centralized & CICIDS2017, NSL-KDD, Kitsune, IoT network intrusion dataset & CNN  & FedAvg & - & 4 & 1-20/1-10 & Accuracy, TPR, FPR &  \\ \hline

%A trusted feature aggregator federated learning for distributed malicious attack detection 
\cite{hei2020trusted} & 2020 & Cross-device & Horizontal & Centralized & KDDCup99 & MLP, DT, SVM, RF  & FedAvg & - & 4 & -/- & Accuracy, Precision, Recall, F1-score, AUC, delay &  \\ \hline

%FIDS: A Federated Intrusion Detection System for 5G Smart Metering Network 
\cite{mirzaee2021fids} & 2021 & Cross-device & Horizontal & Centralized & NSL-KDD & DNN & FedAvg  & - & 16 & 200/50 & Accuracy, Precision, Recall, F1-score, AUC, FPR, delay &  \\ \hline

%Memory efficient federated deep learning for intrusion detection in IoT networks 
\cite{zakariyya2021memory} & 2021 & Cross-device & Horizontal & Centralized & N-BaIoT, Kitsune, IoT-DDoS, WUSTL \cite{teixeira2018scada} & Fully connected NN & FedAvg & Pytorch, Pysyft & 3 & 30/4 & Accuracy, Precision, Recall, F1-score, memory use &  \\ \hline

%FNEL: An Evolving Intrusion Detection System Based on Federated Never-Ending Learning 
\cite{qin2021fnel} & 2021 & Cross-device & Transfer & Centralized & CICIDS2017, CICDDoS2019 & Neural network  & ? & ? & ? & 1-200/1 & Precision, FPR, FNR &  \\ \hline

%FLDDoS: DDoS Attack Detection Model based on Federated Learning
\cite{zhang2021flddos} & 2021  & Cross-device & Horizontal & Centralized & NLSKDD, CICIDS2017, CICDDoS & RNN & Based on FedAvg & Pytorch, Pysyft & 21 & 1-8000/100 & Accuracy, Precision, Recall, F1-score  \\ \hline

%FIDS: Detecting DDoS Through Federated Learning Based Method
\cite{li2021fids} & 2021 & Cross-device & Horizontal & Centralized & CICDDoS2019 & GRU & Based on FedAvg & Pytorch  & 5 & 1-10/200 & Accuracy, loss &  \\ \hline

%Towards Lightweight and Efficient Distributed Intrusion Detection Framework 
\cite{yuan2021towards} & 2021 & Cross-device & Horizontal & Centralized & CICDDoS2019 & GRU & ? & ?  & 1-30 & 1-200/1 & Accuracy, Precision, Recall, F1-score, FPR, communication overhead, time \\ \hline

%A Robust Distributed Intrusion Detection System for Edge of Things
\cite{lalouani2021robust} & 2021 & TO CHECK THIS ONE Cross-device & Horizontal & Centralized & UNSW-NB15-v2 & Neural network & FedAvg & ?  & 10 & 55/1 & Accuracy, Precision, Recall, F1-score, TP &  \\ \hline

%Federated learning-based intrusion detection in SDN-enabled IIoT networks
\cite{duy2021federated} & 2021 & Cross-device & Horizontal & Centralized & CICDDoS2019 & CNN & FedAvg & Flower, TensorFlow Privacy & 3 & 1-10/1 & Accuracy, Precision, Recall, F1-score, communication overhead &  \\ \hline

%Federated transfer learning-based IDS for the internet of medical things (IoMT)
\cite{otoum2021federated} & 2021 & Cross-device & Transfer & Centralized & CICIDS2017 & DNN & FedAvg & Pytorch, TensorFlow & ? & ?/5 & Accuracy, Precision, F1-score, time &  \\ \hline

%Detecting Network Attacks using Federated Learning for IoT Devices 
\cite{shahid2021detecting} & 2021 & Cross-device & Horizontal & Centralized & NSL-KDD & LR, DNN & FedAvg & scikit-learn, PySyft & 4-8 & 1-4/1 & Accuracy, Precision, Recall, F1-score &  \\ \hline

%Towards Fast Network Intrusion Detection based on Efficiency-preserving Federated Learning 
\cite{dong2021towards} & 2021 & Cross-device & Horizontal & Centralized & CIC-DDoS2019 & MLP, Gradient Boosting Decision Tree (GBDT) & Based on FedAvg (DataBin) & Based on Python & 21,66 & 1000-2000/1 & Accuracy, FOR &  \\ \hline

%Trust-based federated learning for network anomaly detection
\cite{chen2021trust} & 2021 & Cross-device & Horizontal & Centralized & KDDCup99 & CNN & Based on FedAvg & Pytorch & 1-20 & 50-300/1 & Accuracy, time &  \\ \hline

%Federated learning for anomaly-based intrusion detection
\cite{ayed2021federated} & Cross-device & Horizontal & Centralized & 2021 & CICIDS2017 & CNN & FedAvg & ? & 10 & 7/10 & Accuracy, loss &  \\ \hline

%A Secure and Privacy Preserving Federated Learning Approach for IoT Intrusion Detection System
\cite{hao2021secure} & 2021 & Cross-device & Horizontal & Centralized & CICIDS2017 & LSTM, NN, CNN & FedAvg & Flask & 2-6 & 3-7/10 & Accuracy, precision, recall, F1 &  \\ \hline

%Federated learning-based intrusion detection in the context of IIoT networks: Poisoning Attack and defense 
\cite{vy2021federated} & 2021 & Cross-device & Horizontal & Centralized & Kitsune & CNN, GRU & FedAvg? & TensorFlow, Keras & 3-9 & 6-12/1 & Accuracy, precision, recall, F1 &  \\ \hline

%Federated deep learning for collaborative intrusion detection in heterogeneous networks 
\cite{popoola2021federated} & 2021 & Cross-silo & Horizontal & Centralized & Ton\_IoT, UNSW-NB15, BoT-IoT, CSE-CIC-CIDS2018 & DNN & FedAvg, CM, Fed+ & - & 4 & 1-10/1-10 & Accuracy, precision, recall, F1-score, MCC &  \\ \hline

%Temporal weighted averaging for asynchronous federated intrusion detection systems 
\cite{agrawal2021temporal} & 2021 & Cross-device & Horizontal & Centralized & NSL-KDD & NN & Temporal Weighted Averaging (proposed) & TensorFlow & 30 & 15/1 & Accuracy, loss &  \\ \hline

%Intrusion Detection based on Privacy-preserving Federated Learning for the Industrial IoT 
\cite{ruzafa2021intrusion} & 2021 & Cross-device & Horizontal & Centralized & Ton\_IoT & LR & FedAvg, Fed+ & IBMFL & 4 & 50/1 & Accuracy, Pearson correlation &  \\ \hline

%Intelligent intrusion detection based on federated learning for edge-assisted Internet of Things 
\cite{man2021intelligent} & 2021 & Cross-device & Horizontal & Centralized & NSL-KDD & CNN & Based on FedAvg (proposed) & Pytorch & 10 & 40-200/40-200 & Accuracy, precision, recall, F1-score &  \\ \hline

%An ensemble multi-view federated learning intrusion detection for iot 
\cite{attota2021ensemble} & 2021 & Cross-device & Horizontal & Centralized & MQTT dataset \cite{MQTT-IoT-IDS2020} & NN & FedAvg & PySyft & 10 & 1-10/1 & Accuracy, precision, recall, F1-score &  \\ \hline

%Adaptive Intrusion Detection in the Networking of Large-Scale LANs With Segmented Federated Learning 
\cite{sun2020adaptive} & 2021 & Cross-device & Horizontal & Centralized & Generated & CNN & FedAvg & - & 20 & 1-60/1 & Accuracy, precision, recall, F1-score &  \\ \hline

%A Blockchain-Based Federated Forest for SDN-Enabled In-Vehicle Network Intrusion Detection System
\cite{aliyu2021blockchain} & 2021 & Cross-device & Horizontal & Centralized & CAN-intrusion dataset (OTIDS) & RF & FedAvg & Based on sklearn & 5-20 & -/- & Accuracy, precision, recall, F1-score &  \\ \hline
 
%LocKedge: Low-Complexity Cyberattack Detection in IoT Edge Computing  
\cite{LocKedge} & 2021 & Cross-device & Horizontal & Centralized & BoT-IoT & NN & FedAvg & Based on Python & 4 & 1000/1 & Acc, Pre, Rec, F1, ROC curve, memory/CPU use &  \\ \hline
 
%Privacy preserving misbehavior detection in IoV using federated machine learning 
\cite{uprety2021privacy} & 2021 & Cross-device & Horizontal & Centralized & Veremi & NN & FedAvg & TensorFlow & 10 & 1-500/1 & Accuracy, precision, recall, communication overhead &  \\ \hline

%Data Privacy Security Guaranteed Network Intrusion Detection System Based on Federated Learning
\cite{shi2021data} & 2021 & Cross-device & Horizontal & Centralized & UNSW-NB15, CICIDS2018 & CNN & FedAvg & - & 10, 15 & 15,20/1 & Accuracy, loss \\ \hline

%Blockchain and Federated Learning for Collaborative Intrusion Detection in Vehicular Edge Computing 
\cite{liu2021blockchain} & 2021  & Cross-device & Horizontal & Decentralized & KDDCup99 & MLP & FedAvg & Pytorch, Pysyft & 2-6 & 10-40/1 & Accuracy, precision, recall  \\ \hline

%Hierarchical Federated Learning for Collaborative IDS in IoT Applications 
\cite{saadat2021hierarchical} & 2021 & Cross-device & Horizontal & Centralized & NSLKDD & NN & FedSGD, FedAvg & - & 4-8 & 1-20/1 & Accuracy, loss \\ \hline

%DeepFed: Federated Deep Learning for Intrusion Detection in Industrial Cyber--Physical Systems 
\cite{li2020deepfed} & 2021 & Cross-device & Horizontal & Centralized & \cite{morris2014industrial} & CNN, GRU, MLP & FedAvg & Flask, Keras & 3-7 & 2-10/1 & Accuracy, precision, recall, F1-score &  \\ \hline

%IDS for industrial applications: a federated learning approach with active personalization 
\cite{kelli2021ids} & 2021 & Cross-device & Horizontal & Centralized & Generated & Neural network & FedAvg & - & 3 & 1-3/1 & Accuracy, precision, F1-score &  \\ \hline

%\hl{Security and privacy-aware artificial intrusion detection system using federated machine learning}  
\cite{kumar2021security} & 2021 & KDD99Cup & ? & ? & - & ? & ?-?/1 &  &  \\ \hline

%On-device Malware Detection using Performance-Aware and Robust Collaborative Learning
\cite{shukla2021device} & 2021 & Cross-device & Horizontal & Centralized & Generated from VirusTotal & CNN, RF, LR, KNN & Based on FedProx & ? & 10-50 & 200/20-40 & Accuracy, time, power, energy  \\ \hline

%Train Me to Fight: Machine-Learning Based On-Device Malware Detection for Mobile Devices
\cite{pasdar2022train} & 2022 & Cross-silo & Transfer & Centralized & Maldroid, Drebin, AndroZoo & CNN & FedAvg & TensorFlow Lite, keras & 3 & 1-4000/1-8000 & Accuracy, loss, F1, time, CPU, memory  \\ \hline

%DDoS Attack Detection Based on CNN and Federated Learning
\cite{lv2022ddos} & 2022 & Cross-device & Horizontal & Centralized & CICDDoS-2019 & CNN & FedAvg & Pytorch & 50 & 1-1000/1 & Accuracy, precision, recall, F1-score &  \\ \hline

%Grid False Data Intrusion Detection Method Based on Edge Computing and Federated Learning
\cite{zhang2022grid} & 2022 & Cross-device & Horizontal & Centralized & Generated & CNN-LSTM & FedAvg? & - & 4 & ?/? & Accuracy  &  \\ \hline

%Detection DDoS of Attacks Based on Federated Learning with Digital Twin Network
\cite{su2022detection} & 2022 & Cross-device & Horizontal & Centralized & KDDCup99 & LSTM & FedAvg, Based on FedProx & Based on Python & ? & 1-200/1-20 & Accuracy, precision, recall, F1  \\ \hline

%Dew-Cloud-Based Hierarchical Federated Learning for Intrusion Detection in IoMT
\cite{singh2022dew} & 2022 & Cross-device & Horizontal & Centralized & NSL-KDD, Ton\_IoT & LSTM & Based on FedAvg (hierarchical) & Keras, Scikit-learn, TensorFlow, Numpy & ? & 1-100/1 & Accuracy, precision, recall, F1 &  \\ \hline

%Federation Learning for Intrusion Detection Methods by Parse Convolutional Neural Network
\cite{luo2022federation} & 2022 & Cross-device & Horizontal & Centralized & NSL-KDD & CNN & FedAvg & Pytorch & ? & ?/? & Accuracy, Recall, FPR, time  \\ \hline

%Federation Learning of Optimized Convolutional Neural Network Structure for Intrusion Detection
\cite{yang2022federation} & 2022 & Cross-device & Horizontal & Centralized & NSL-KDD & CNN & FedAvg & Pytorch & ? & ?/? & Accuracy, Recall, FPR, time   \\ \hline

%Random Forest Based on Federated Learning for Intrusion Detection
\cite{markovic2022random} & 2022 & Cross-device & Horizontal & Centralized & KDD,NSL-KDD, UNSW-NB15, CIC-IDS-2017 & RF & FedAvg & ? & 3-14 (depending on the dataset) & ? & Accuracy  \\ \hline

%FeCo: Boosting Intrusion Detection Capability in IoT Networks via Contrastive Learning 
\cite{wang2022feco} & 2022 & Cross-device & Horizontal & Centralized & NSL-KDD & NN & FedAvg & Pytorch & 50 & 15/4 & Accuracy, recall, precision, F1, FPR, time  \\ \hline

%Intrusion Detection for Maritime Transportation Systems With Batch Federated Aggregation 
\cite{liu2022intrusion} & 2022 & Cross-device & Horizontal & Centralized & NSL-KDD & CNN-MLP & FedBatch (proposed) & Pytorch & 100 & \hl{?} & Accuracy, precision, recall F1-score &  \\ \hline

%A federated learning framework for cyberattack detection in vehicular sensor networks 
\cite{driss2022federated} & 2022 & Cross-device & Horizontal & Centralized & Car Hacking \cite{qvr7-n418-21} & RF, GRU & FedAvg & TensorFlow, Keras & ? & ?-100 & Accuracy, precision, recall F1-score, time  \\ \hline

%A Robust Distributed Intrusion Detection System for Collusive Attacks on Edge of Things
\cite{lalouani2022robust} & Cross-device & Horizontal & Centralized & 2021 & UNSW-NB15-v2 & NN & FedAvg & ?  & 10 & 1-18/1 & Accuracy, Precision, Recall, F1-score\\ \hline

%Federated Learning for Privacy Preservation of Healthcare Data from Smartphone-based Side-Channel Attacks
\cite{rehman2022federated} & 2022 & Cross-silo & Horizontal & Centralized & Generated (Based on \cite{javed2020alphalogger}) & DNN & FedAvg & ? & 2 & 1-3/20 & Accuracy, precision, recall, F1, loss, ROC &  \\ \hline

%On the Feasibility of Split Learning, Transfer Learning and Federated Learning for Preserving Security in ITS Systems
\cite{otoum2022feasibility} & 2022 & Cross-device & Horizontal & Centralized & CICIDS2017 & NN & FedAvg & sklearn & 1-100 & 1-10/1 & Accuracy, DR, power consumption  \\ \hline

%Edge-IIoTset: A New Comprehensive Realistic Cyber Security Dataset of IoT and IIoT Applications for Centralized and Federated Learning 
\cite{ferrag2022edge} & 2022 & Cross-device & Horizontal & Centralized & Edge-IIoTset (proposed) & DT, RF, KNN, SVM, DNN & FedAvg & Based on sklearn  & 5-15 & 1-10/1 & Accuracy \\ \hline


%PEFL: Deep Privacy-Encoding-Based Federated Learning Framework for Smart Agriculture 
\cite{kumar2021pefl} & 2022 & Cross-device & Horizontal & Centralized & Ton\_IoT & GRU & FedAvg? & PySyft  & 2 & 1-100/1-100 & Accuracy, precision, F1, Detection Rate (DR) &  \\ \hline

%Evaluating Federated Learning for intrusion detection in Internet of Things: Review and challenges
\cite{campos2021evaluating} & 2022 & Cross-device & Horizontal & Centralized  & Ton\_IoT & LR & FedAvg, Fed+ & IBMFL  & 4-10 & 1-300/1 & Accuracy, precision, recall, F1, FPR  &  \\ \hline

%Federated Learning-based Anomaly Detection for IoT Security Attacks 
\cite{mothukuri2021federated} & 2022 & Cross-device & Horizontal & Centralized & \cite{frazao2018denial} & LSTM, GRU & FedAvg & Pytorch, Pysyft  & 1-40 & ?/? & Accuracy, precision, recall, F1, time &  \\ \hline

%Improving detection of scanning attacks on heterogeneous networks with Federated Learning
\cite{de2022improving} & 2022 & Cross-device & Horizontal & Centralized & Ton\_IoT & LR & FedAvg & sklearn  & 13 & 50/10 & F1  \\ \hline

%Federated transfer learning with client selection for intrusion detection in mobile edge computing
\cite{cheng2022federated} & 2022 & Cross-device & Transfer & Centralized & NSL-KDD, UNSW-NB15 & CNN & FedSGD & Pytorch, Pysyft  & 10 & 1-40/1 & Accuracy  \\ \hline

%Federated intrusion detection in blockchain-based smart transportation systems
\cite{abdel2021federated} & 2022 & Cross-device & Horizontal & Centralized & Car Hacking \cite{qvr7-n418-21}, Ton\_IoT & Transformer & FedAvg & PySyft  & 20 & 30/50 & Accuracy, precision, recall, F1 &  \\ \hline

%A federated learning framework for detecting false data injection attacks in solar farms
\cite{zhao2021federated} & 2022 & Cross-device & Horizontal & Centralized  & Generated & LSTM & FedAvg & Flower, Pytorch  & 3 & 300/1 & Accuracy, precision, recall, F1, loss, time, communication overhead &  \\ \hline

%Federated Deep Learning for Zero-Day Botnet Attack Detection in IoT Edge Devices
\cite{popoola2021federated} & 2022 & Cross-device & Horizontal & Centralized & BoT-IoT, N-BaIoT & DNN & FedAvg & IBMFL, TensorFlow, Keras  & 5 & 1-8/5 & Accuracy, precision, recall, F1, time, memory  \\ \hline

%FedLearnSP: preserving privacy and security using federated learning and edge computing
%\cite{makkar2021fedlearnsp} & 2022 & \cite{makkar2020spami} & CNN & FedAvg? & ? & 5 & ?/? & TPR, FPR, TP, FP, TN, FN, time
 &  \\ \hline

%Federated Learning for Intrusion Detection in the Critical Infrastructures: Vertically Partitioned Data Use Case
\cite{novikova2022federated} & 2022 & Cross-device & Vertical & Centralized & SWaT \cite{goh2016dataset} & GBDT & SecureBoost? & FATE & 6 & ?/? & Accuracy, time &  \\ \hline

%Differentially private self-normalizing neural networks for adversarial robustness in federated learning
\cite{ibitoye2022differentially} & 2022 & Cross-device & Horizontal & Centralized & MNIST, CTU-13 & CNN & FedAvg & TensorFlow, IBMFL & 200 & ?/? & Accuracy, time &  \\ \hline

%A federated learning method for network intrusion detection
\cite{tang2022federated} & 2022 & Cross-device & Horizontal & Centralized & CICIDS2017 & GRU & FedAvg & Pytorch, Pysyft & 2 & 1-500/1 & Accuracy, precision, recall, F1 &  \\ \hline

%RAFeL - Robust and Data-Aware Federated Learning-inspired Malware Detection in Internet-of-Things (IoT) Networks
\cite{shukla2022rafel} & 2022 & Cross-device & Horizontal & Centralized & Generated & CNN, Mobile-Net, RF, LR, KNN, MLP & Based on FedProx & ? & 10-50 & 200/20-40 & Accuracy, power, energy, and area on-chip &  \\ \hline

%FELIDS: Federated learning-based intrusion detection system for agricultural Internet of Things
\cite{friha2022felids} & 2022 & Cross-device & Horizontal & Centralized & CICIDS2018, InSDN \cite{elsayed2020insdn}, MQTTset \cite{vaccari2020mqttset}
& DNN, CNN, RNN & FedAvg & Sherpa.ai, TensorFlow, Keras & 5-15 & 1-50/1 & Accuracy, precision, recall, F1, time, energy &  \\ \hline

%FEDGAN-IDS: Privacy-preserving IDS using GAN and Federated Learning
\cite{tabassum2022fedgan} & TO CHECK THIS ONE 2022 & Cross-device & Horizontal & Centralized & NSL-KDD, KDD-CUPP99, UNSW-NB15 & CNN & FedAvg & ? &? & 1-30/1-200 & Accuracy, precision, recall, F1, AUC &  \\ \hline
  
%SecFedNIDS: Robust defense for poisoning attack against federated learning-based network intrusion detection system
\cite{zhang2022secfednids} & 2022 & Cross-device & Horizontal & Centralized & UNSW-NB15, CICIDS2018 & CNN & FedAvg* & Pytorch & 100 & 1-50/1 & Accuracy, recall &  \\ \hline

%Experience-Driven Attack Design and Federated-Learning-Based Intrusion Detection in Industry 4.0
\cite{tahir2021experience} & 2022 & Cross-device & Horizontal & Centralized & Based on \cite{nreldataset} & GRU & FedAvg, Fed-AA, DeepFed-Avg, DeepFed-AA & Matpower, Pytorch & ? & 1-50/1 & Accuracy, precision, recall, F1, time &  \\ \hline

%A Hierarchical Federated Learning-Based Intrusion Detection System for 5G Smart Grids
\cite{sun2022hierarchical} & 2022 & Cross-device & Horizontal & Centralized & NSL-KDD & MLP, CNN & FedAvg & TensorFlow & 10 & 1-100/1-10 & Accuracy, precision, F1, overhead &  \\ \hline


\end{longtable}
%}
\end{center}
\twocolumn
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%55
%\end{tabular}
%\caption{Classification of existing works on FL-enabled IDS based on supervised models}
%\label{tab:super_taxonomy_table}
%\end{table*}
%\end{landscape}

==> unsuperv-table.tex <==
\onecolumn
\begin{center}
\tiny
%\fontsize{6}{11}\selectfont{
\begin{longtable}{C{0.4cm}C{0.4cm}C{1.2cm}C{1.2cm}C{1.2cm}C{1.5cm}C{1.5cm}C{1.5cm}C{1.5cm}C{0.8cm}C{0.8cm}C{2.5cm}}
\caption{Classification of existing works on FL-enabled IDS based on semi-supervised and unsupervised models}
\label{tab:super_taxonomy_long_table} \\

%\textbf{Training rounds/epochs}
\hline 
\textbf{Ref.} & \textbf{Year} & \textbf{Network Architecture} & \textbf{Data Availability} & \textbf{Data Partitioning} & \textbf{Dataset} & \textbf{ML Model} & \textbf{Aggregation function} & \textbf{FL implementation}  & \textbf{Training parties} & \textbf{Training rounds} & \textbf{Evaluation metrics} \\
\hline 
\endfirsthead

\multicolumn{12}{c}%
%{{\bfseries \tablename\ \thetable{} -- continued from previous page}} \\
{\tablename\ \thetable{} -- continued from previous page} \\
\hline 
\textbf{Ref.} & \textbf{Year} & \textbf{Network Architecture} & \textbf{Data Availability} & \textbf{Data Partitioning} & \textbf{Dataset} & \textbf{ML Model} & \textbf{Aggregation function} & \textbf{FL implementation}  & \textbf{Training parties} & \textbf{Training rounds} & \textbf{Evaluation metrics} \\
\hline 
\endhead

\hline \multicolumn{12}{c}{{Continued on next page}} \\ \hline
\endfoot

\hline \hline
\endlastfoot

%Chained Anomaly Detection Models for Federated Learning: An Intrusion Detection Case Study
\cite{preuveneers2018chained} & 2018 & Cross-device & Horizontal & Centralized & CICIDS2017 & Autoencoders  &  FedAvg & Based on Keras, Deeplearning4j and Spring Boot 2.0 & 2-12 & 1/1-50 & Accuracy, loss, time &  \\ \hline

%Federated wireless network intrusion detection 
\cite{cetin2019federated} & 2019 & Cross-device & Horizontal & Centralized &  AWID & Stacked Autoencoders & FedAvg & LEAF & 933 & 1-20/1 & Accuracy, communication overhead &  \\ \hline


%FED-IIoT: A Robust Federated Malware Detection Architecture in Industrial IoT
\cite{taheri2020fed} & 2020 & Cross-device & Horizontal & Centralized & Drebin \cite{arp2014drebin}, \cite{zhou2012dissecting}, \cite{Contagio} & GAN based on CNN &  FedAvg, Krum & TensorFlow, Keras & 5-15 & 1-300/1-300 & Accuracy &  \\ \hline

%Network anomaly detection using federated deep autoencoding Gaussian mixture model
\cite{gaussian2020network} & 2020 & Cross-silo & Horizontal & Centralized & KDD99Cup & Deep autoencoding gaussian mixture model &  FedAvg & - & 2 & 1-60/1 & Precision, recall, F1-score &  \\ \hline

%Collaborative learning model for cyberattack detection systems in iot industry 4.0
\cite{khoa2020collaborative} & 2020 & Cross-device & Horizontal & Centralized & KDD, NSLKDD, UNSW-NB15, N-BaIoT & DBN  & - & FedAvg & 2, 3 & -/- & Accuracy, precision, TPR &  \\ \hline

%Deep Federated Learning-Based Cyber-Attack Detection in Industrial Control Systems
\cite{jahromi2021deep} & 2021 & Cross-device & Horizontal & Centralized & SWaT & Stacked autoencoders & FedAvg & - & - & -/- & Accuracy, precision, recall, F1 &  \\ \hline

%Unsupervised Federated Learning based IoT Intrusion Detection 
\cite{yadav2021unsupervised} & 2021 & Cross-device & Horizontal & Centralized & CICIDS2017 & AE, NN & FedAvg & -  & - & 1-100/1-100 & Accuracy, MSE &  \\ \hline

%Property Inference-based Federated Learning Groups for Collaborative Network Anomaly Detection 
\cite{wettlaufer2021property} & 2021 & Cross-device & Horizontal & Centralized & CICIDS2017 & Elliptic Envelope, Isolation Forest & FedAvg? & - & - & 5/1 & Accuracy, F1-score &  \\ \hline

%An Architecture for Federated Learning Enabled Collaborative Intrusion Detection System
\cite{mcosker2021architecture} & 2021 & Cross-device & Horizontal & Centralized & CICIDS2017 & SOM & FedAvg? & PySyft & - & -/- & Accuracy, precision, recall F1-score &  \\ \hline

%An Improved K-Means Clustering Intrusion Detection Algorithm for Wireless Networks Based on Federated Learning
\cite{xie2021improved} & 2021 & Cross-device & Horizontal & Centralized & AWID & K-means clustering & FedAvg & Based on Python & 10 & 2-10/1 & Accuracy, FAR &  \\ \hline

%Clustering based Rewarding Algorithm to Detect Adversaries in Federated Machine Learning based IoT Environment
\cite{yadav2021clustering} & 2021 & Cross-device & Horizontal & Centralized & NSL-KDD & Based on K-means & FedAvg & Based on Python & 10 & 1-100/1 & Accuracy, WCSS &  \\ \hline

%Federated Deep Learning Approaches for the Privacy and Security of IoT Systems 
\cite{alazzam2022federated} & 2022 & Cross-device & Horizontal & Centralized & Generated & AE & FedAvg? & Pytorch & ? & ? & Accuracy, precision, recall, F1, FPR, FNR, memory use &  \\ \hline

%Fed\_ADBN: An efficient intrusion detection framework based on client selection in AMI network 
\cite{xia2022fed_adbn} & 2022 & Cross-device & Horizontal & Centralized & NSL-KDD & DBN & FedAvg & TensorFlow  & 100 & 1-30/30-50 & Accuracy, precision, recall, F1, time &  \\ \hline

%Federated Learning for Malware Detection in IoT Devices
\cite{rey2022federated} & 2022 & Cross-device & Horizontal & Centralized & N-BaIoT & MLP, autoencoders & FedAvg, Coordinate-wise median/trimmed mean & Own library  & 8 & 1-29/1-4 & Accuracy, F1, FPR, TPR &  \\ \hline

%Anomaly Detection in Multi-Host Environment Based on Federated Hypersphere Classifier 
\cite{kwon2022anomaly} & TO CHECK THIS 2022  & Cross-device & Horizontal & Centralized & MNIST, CIFAR-10, CICIDS-2017, TON\_IoT & K-means clustering & FedAvg & Based on Pytorch & ? & ? & AUC, F1&  \\ \hline

%Privacy-preserving knowledge transfer for intrusion detection with federated deep autoencoding gaussian mixture model 
\cite{chen2022privacy} & 2022  & Cross-silo & Horizontal & Centralized & KDDCUP99, NSL-KDD, CSE-CIC-IDS2017, CSE-CIC-IDS2018  & AE & FedAvg & ? & 2 & 1-120/200 & Precision, recall, F1  \\ \hline

\multicolumn{12}{c}{Based on semi-supervised models}
\\ \hline
%FLUIDS: Federated Learning with semi-supervised approach for Intrusion Detection System Open Access 
\cite{aouedi2022fluids} & 2022 & Cross-device & Horizontal & Centralized & UNSW-NB15 & AE-NN  & FedAvg & Pytorch & 100 & 6/5 & F1 &  \\ \hline

%Federated Semi-Supervised Learning for Attack Detection in Industrial Internet of Things 
\cite{aouedi2022federated} & 2022 & Cross-device & Horizontal & Centralized & \cite{morris2014industrial} & AE-NN  & FedAvg & Pytorch & 100 & 18/20-100 & Accuracy, precision, recall, F1, communication overhead &  \\ \hline

%A Knowledge Transfer-based Semi-Supervised Federated Learning for IoT Malware Detection
\cite{pei2022knowledge} & 2022 & Cross-device & Transfer & Centralized & Drebin, MalDroid, AndroZoo, VirusShare & SACN & FedAvg & Keras & 100-500 & ?/? & FPR, TPR, ROC curve, F1-score  \\ \hline

%Semi-Supervised Federated Learning Based Intrusion Detection Method for Internet of Things
\cite{zhao2022semi} & 2022 & Cross-device & Horizontal & Centralized & N-BaIoT & CNN & FedAvg & Pytorch & 27, 89 & 1-200/100 & Accuracy, precision, F1-score, communication overhead  \\ \hline

\end{longtable}
%}
\end{center}
\twocolumn
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%55
%\end{tabular}
%\caption{Classification of existing works on FL-enabled IDS based on supervised models}
%\label{tab:super_taxonomy_table}
%\end{table*}
%\end{landscape}


